Prompt Tuning for Zero-shot Compositional Learning

Open World Compositional Zero-Shot Learning (OW-CZSL) is known to be an extremely challenging task, which aims to recognize unseen compositions formed from seen attributes and objects without any prior assumption of the output space. In order to achieve this goal, a model has to be "smart" and "knowledgeable". To be smart, a model should be good at reasoning the interactions between attributes and objects from the seen compositions. While "knowledgeable" means the model owns "common sense" to the open world that can "foresee" some features of the unseen compositions. Most previous work focuses on the "smart" part, while few of them provided an effective solution to achieve the "knowledgeable" goal. In this paper, we proposed a framework named Multi-Modal Prompt Tuning (MMPT) to inherit the "knowledgeable" property from the large pre-trained vision-language model. Extensive experiments show that our proposed MMPT obtains new state-of-the-art results in OW-CZSL task. On the UT-Zappos dataset, MMPT pushes the AUC score to $29.8$, while the previous best score is $26.5$. On the more challenging MIT-States dataset, the AUC score of MMPT is 1.5 times better than the current state-of-the-art.

==> fig_tab_tex/case_mit.tex <==
\begin{figure} [htbp]
  \raggedleft
   \includegraphics[width=\columnwidth]{figures_tmp/casestudy_mit.png}
       \caption{Top-5 prediction results of MMPT and EpiCA \cite{xu-etal-2021-zero}。
       }
    \label{fig:casestudy_mit}
\end{figure}

==> fig_tab_tex/case_mit_retrival.tex <==
\begin{figure*} [htbp]
  \raggedleft
   \includegraphics[width=\textwidth]{figures_tmp/casestudy_mit_retrieval.png}
       \caption{Image retrieval results by MMPT and KG-SP \cite{karthik2022kg-sp}
       }
      \label{fig:casestudy_mit_retrieval}
\end{figure*}

==> fig_tab_tex/intro_fig.tex <==
\begin{figure} [htbp]
  \raggedleft
   \includegraphics[width=\columnwidth]{figures_tmp/intro_task.png}
       \caption{Examples of Compositional Zero-shot Learning (CZSL). The left panel contains are examples of seen composition in the training set, while the right panel shows the unseen compositions in the testing set. 
       }
    \label{fig:intro}
\end{figure}

==> tab_temp/comparison_params_table.tex <==


\section{Shared prompt embedding dimension}
MIT testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Shared prompt dim 64 &  33.0  &    17.5 &  14.8  &  4.0  \\
  Shared prompt dim 128 &  \textbf{32.6}  &  \textbf{18.2}   &  \textbf{15.0}   &  \textbf{4.1} \\
   Shared prompt dim 256 & 35.1  &  17.0   &   15.3 &   4.3  \\
    Shared prompt dim 512 &  34.7 &  17.3   & 15.0   &  4.2   \\
 \hline
\end{tabular}
UT-zappos testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Shared prompt dim 64 & 62.2  &     57.1& 45.5   & 29.5    \\
  Shared prompt dim 128 & \textbf{63.1}   &  \textbf{56.6}   &  \textbf{45.4}  &  \textbf{30.0}  \\
   Shared prompt dim 256 & 60.8  &  53.4   & 41.0   & 25.8    \\
    Shared prompt dim 512 & 63.7  &  57.1   &  46.2  &  30.2    \\
 \hline
\end{tabular}

\section{Number of ctx token}
MIT testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Ctx 1 &  31.1 & 18.2  & 15.2  & 4.1  \\
 Ctx 2 & 33.2  &  16.8   &  14.7  &  3.9  \\
  Ctx 4 & \textbf{32.6}  &  \textbf{18.2}   &  \textbf{15.0}   &  \textbf{4.1}  \\
   Ctx 6 &   34.2 &  17.4   & 15.0   &    4.1  \\
    Ctx 8 & 33.5  &  17.3   &  14.7  &  4.1  \\
 \hline
\end{tabular}



UT-zappos testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
  Ctx 1 & 66.2  & 53.1  & 43.5  &  28.9  \\
  Ctx 2 & 66.5 &  54.0   & 45.8   &  30.2  \\
  Ctx 4 & \textbf{63.1}   &  \textbf{56.6}   &  \textbf{45.4}  &  \textbf{30.0}  \\
   Ctx 6 & 61.5 &   55.8  &  44.0  & 28.4  \\
    Ctx 8 & 60.8  & 55.3    &  44.6  & 28.3  \\
 \hline
\end{tabular}

\section{Depth of prompt layer }
MIT testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
  Depth 2 &   &   &   &   \\
  Depth 4 &  29.9 & 18.2  &  14.4 &  3.8 \\
 Depth 9 &  \textbf{32.6}  &  \textbf{18.2}   &  \textbf{15.0}   &  \textbf{4.1}  \\
 Depth 12 &   &   &   &   \\
 \hline
\end{tabular}

UT-zappos testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Depth 2 & 60.9 & 55.4 & 43.8 & 27.9   \\
 Depth 4 & 63.4 & 56.7    & 44.8 &  29.3 \\
  Depth 6 &  63.4 & 56.5 & 46.1 & 30.3\\
  Depth 9 & \textbf{63.1}   &  \textbf{56.6}   &  \textbf{45.4}  &  \textbf{30.0}  \\
  Depth 12 &  60.0 & 53.7  & 43.4  &  26.9  \\
 \hline


\end{tabular}



==> tab_temp/comparison_params_table_withoutknowledge.tex <==
\pagebreak
\section{Shared prompt embedding dimension}
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Shared prompt dim 64 &   33.5  & 16.8   & 14.4  &  3.9  \\
  Shared prompt dim 128 &  33.5 &   17.3  &  14.9  &  4.1  \\
   Shared prompt dim 256 &  35.6 & 16.3  &  14.9  &  4.2  \\
    Shared prompt dim 512 & 35.4 &  16.6  & 14.7   &   4.1 \\
 \hline
\end{tabular}
\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Shared prompt dim 8 & 63.4 & 54.0 & 44.9 & 28.9 \\
 Shared prompt dim 16 & 61.8 & 55.5 & 44.7 & 28.6 \\
 Shared prompt dim 32  & 65.1 & 55.7 & 46.5 & 30.5 \\
 Shared prompt dim 64 & 62.0 & 57.6  &  45.6  &  29.6   \\
  Shared prompt dim 128 &  63.3 &  56.0   &  45.1  &  29.8  \\
   Shared prompt dim 256 &  61.0 &  53.7   &  41.1  &  26.0  \\
    Shared prompt dim 512 &  63.5 &  56.4   &  45.7  &   29.8 \\
 \hline
\end{tabular}

\section{Number of ctx token}
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Ctx 1 & 31.8  & 17.8  & 14.9  & 4.0  \\
 Ctx 2 &  35.3 &  15.3   &  14.0  & 3.7   \\
  Ctx 4 &  33.5 &   17.3  &  14.9  &  4.1  \\
   Ctx 6 &  35.8 &  15.4   & 13.9 &  3.8  \\
    Ctx 8 &  36.3  & 15.4    &  14.3  &  3.9  \\
 \hline
\end{tabular}
\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
  Ctx 1 & 65.7  &   53.0  &  43.6  &  28.6  \\
  Ctx 2 & 65.6  &  53.7   &  46.2  &  30.1  \\
  Ctx 4 &  63.3 &  56.0   &  45.1  &  29.8  \\
   Ctx 6 & 61.5  &  55.7   &  44.6  &  28.5  \\
    Ctx 8 & 61.2  &  55.3   &  44.3  &  28.3  \\
 \hline
\end{tabular}

\section{Depth of prompt layer }
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 Depth 2 & 29.7  &  17.2   & 13.9  &  3.6  \\
 Depth 4 &  34.1 &  16.5   &  14.7  &  4.0  \\
  Depth 6 & 33.7  &  16.6   &  14.8  & 3.9   \\
  Depth 9 & 33.5 &   17.3  &  14.9  &  4.1  \\
  Depth 12 &  37.1 &  15.7   &  14.4  &  4.0  \\
 \hline
\end{tabular}
\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
  Depth 2 & 60.9  &  54.6 & 43.1  &  27.5 \\
  Depth 4 & 63.4  &  56.2   & 44.3   &  29.0  \\
    Depth 6 & 60.3  & 55.2  & 44.3  & 28.2  \\
 Depth 9 & 63.3 &  56.0   &  45.1  &  29.8 \\
 Depth 12 & 59.7  &  53.3 &  43.2 &  26.7 \\
 \hline
\end{tabular}
\\



\section{Visual patch prompt}
MIT testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 No visual patch  & 36.3 & 16.3 & 14.7 & 4.1 \\
 With visual patch & 33.5 &   17.3  &  14.9  &  4.1  \\
 \hline
\end{tabular}
\\
UT-zappos testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results without knowledge} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 No visual patch  & 63.8  &  54.5   & 44.5   &  28.9  \\
 With visual patch & 63.3 &  56.0   &  45.1  &  29.8 \\
 \hline
\end{tabular}



\section{CoOp style no visual patch}
MIT testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
CoOp style no visual patch  & 33.5 &  16.8 & 14.4 & 3.9 \\
 Basic-4-Shared prompt &  33.5 &   17.3  &  14.9  &  4.1   \\
 \hline
\end{tabular}
\\
UT-zappos testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
CoOp style no visual patch  & 60.2  & 50.0    & 41.5  & 25.0  \\
  Basic-4-Shared prompt  & 63.3  &  56.0  &  45.1  &  \textbf{29.8}  \\
 \hline
\end{tabular}

==> tab_temp/main-res-1111tmp.tex <==
\begin{table*}[!htp]\centering
\caption{Open World CZSL results on UT-Zappos and MIT-states. The  best seen (S) and unseen accuracy (U), best harmonic mean (HM), and area under the curve (AUC) are reported on the test sets of the two datasets. \thua{add cite}}
\label{tab:main-res-1111tmp}
\begin{tabular}{l|rrrr|rrrrr}\toprule
\
&\multicolumn{4}{c}{UT-Zappos Test} &\multicolumn{4}{c}{MIT-states test} \\\cmidrule{2-9}
&S &U &HM &AUC &S &U &HM &AUC \\\midrule
LE+ &60.4 &36.5 &30.5 &16.3 &14.2 &2.5 &2.7 &0.3 \\
VisProd &54.6 &42.8 &36.9 &19.7 &20.9 &5.8 &5.6 &0.7 \\
SymNet &53.3 &44.6 &34.5 &18.5 &21.4 &7 &5.8 &0.8 \\
AoP &50.9 &34.2 &29.4 &13.7 &16.6 &5.7 &4.7 &0.7 \\
TMN &55.9 &18.1 &21.7 &8.4 &12.6 &0.9 &1.2 &0.1 \\
CompCos &59.3 &46.8 &36.9 &21.3 &25.4 &10 &8.9 &1.6 \\
KG-SP &61.8 &52.1 &42.3 &26.5 &28.4 &7.5 &7.4 &1.3 \\ \hline
{CLIP} &{{54.7}}	&{{45.7}}	& {35.9}	& {20.0} & {27.9}  & {16.9}  & {13.6}  & {3.3 }\\

(Ours) &\textbf{63.3} &\textbf{56.0} &\textbf{45.1} &\textbf{29.8} & \textbf{32.6} &\textbf{17.7} &\textbf{15.0} &\textbf{4.1} \\

\bottomrule
\end{tabular}
\end{table*}



			

==> tab_temp/result_table.tex <==
\section{MIT-states}

Comparison of backbone architecture on validation set.\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT-states validation results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
  (State-of-the-art) KG-SP   & 29.9   & 7.7 &  8.3 & 1.5\\
KG-SP with CLIP-ViT-backbone  & \textbf{37.1}   & 16.7 &  14.8 & 4.2\\ % step-20
(Ours) Basic-2   & 32.5 & \textbf{18.9}  &  \textbf{16.1}  & \textbf{4.5}  \\ % step-20
 (Ours) Basic-4-Shared-Prompt   & \textbf{37.3}  &  \textbf{17.2}   &  \textbf{16.1}   &  \textbf{4.7}  \\ % step-80 
 \hline
\end{tabular}
\\
\\
Comparison of backbone architecture on testing set.\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT-states testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 (State-of-the-art) KG-SP  & 28.4   & 7.5 &  7.4 & 1.3\\
KG-SP with CLIP-ViT-backbone  & \textbf{37.9}   & 16.1 &  14.7 & 4.1\\
  (Ours) Basic-2   & 34.5 & \textbf{17.8}  &  \textbf{15.0}  & \textbf{4.2}  \\ 
 (Ours) Basic-2 wo knowledge   & 35.4  & 17.0 & 14.9 & 4.2  \\ 
  (Ours) Basic-4-Shared-Prompt   & \textbf{32.6}  &  \textbf{18.2}   &  \textbf{15.0}   &  \textbf{4.1}  \\ 
 \hline
\end{tabular}

\section{UT-Zappos}
Comparison of backbone architecture on validation set.\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-Zappos validation results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 (State-of-the-art) KG-SP  & 61.4   & 58.9 & 34.6  & 21.8 \\
KG-SP with CLIP-ViT-backbone  & 63.6  & 60.9  & 35.1  & 23.3 \\
 (Ours) Basic-2-step-40   & \textbf{63.6} & \textbf{62.1}  &  \textbf{39.0 }  & \textbf{26.5}  \\ % step-40
  (Ours) Basic-Remove-Text-Instruction   &  48.8 & 60.9   &  29.6   &  16.3 \\ % step-160
    (Ours) Basic-4-Shared-Prompt   & \textbf{66.0}  &  \textbf{63.4}   &  \textbf{42.2}   &  \textbf{29.2}  \\ % 
 \hline
\end{tabular}

Comparison of backbone architecture on testing set.\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-Zappos testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 (State-of-the-art) KG-SP  &  61.8 &  52.1 & 42.3  & 26.5 \\
KG-SP with CLIP-ViT-backbone  & 61.7  & 48.1   & 40.8 & 24.8  \\ %1104 in progress
(Ours) Basic-2   & \textbf{65.5} & \textbf{56.3}  &  \textbf{45.6}  & \textbf{30.8}  \\ 
 (Ours) Basic-2 wo knowledge   &  65.2  & 55.6  & 45.0 &  30.3 \\ 
 (Ours) Basic-Remove-Text-Instruction  & 58.8   &  48.4   &  39.2  &  22.9  \\ 
 (Ours) Basic-4-Shared-Prompt   & \textbf{63.1}   &  \textbf{56.6}   &  \textbf{45.4}  &  \textbf{30.0}  \\ 
 (Ours) Basic-4-Shared-Prompt wo knowledge   &  62.9   &  55.6   &  45.0  &  29.3   \\ 
 \hline
 \hline
\end{tabular}

\section{AO-Clever}
Comparison with other model on testing set.\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{AO-Clever testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 (State-of-the-art) {2206.00415 paper} & 97.1  & 99.3 & 95.1 & 95.6 \\
  (Ours) Basic-4-Shared-Prompt   & \textbf{99.9}  & \textbf{99.9}  &  \textbf{97.2}  & \textbf{99.1}  \\ 
 \hline
\end{tabular}



==> tab_temp/visual_patch_table.tex <==
\section{Visual patch prompt}
MIT testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{MIT testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 No visual patch  & & & & \\
 With visual patch &  \textbf{32.6}  &  \textbf{18.2}   &  \textbf{15.0}   &  \textbf{4.1}  \\
 \hline
\end{tabular}
\\
UT-zappos testing results\\
\begin{tabular}{|c|c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{UT-zappos testing results} \\
 \hline
Models & S & U & HM & AUC \\
 \hline
 No visual patch  & 63.8 &  54.5 & 44.5 & 28.9 \\
 With visual patch & \textbf{63.1}   &  \textbf{56.6}   &  \textbf{45.4}  &  \textbf{30.0}  \\
 \hline
\end{tabular}

